Investigating Table-to-Text Generation Capabilities of LLMs in Real-World Information Seeking Scenarios

Tabular data is prevalent across various industries, necessitating significant time and effort for users to understand and manipulate for their information-seeking purposes. The advancements in large language models (LLMs) have shown enormous potential to improve user efficiency. However, the adoption of LLMs in real-world applications for table information seeking remains underexplored. In this paper, we investigate the table-to-text capabilities of different LLMs using four datasets within two real-world information seeking scenarios. These include the LogicNLG and our newly-constructed LoTNLG datasets for data insight generation, along with the FeTaQA and our newly-constructed F2WTQ datasets for query-based generation. We structure our investigation around three research questions, evaluating the performance of LLMs in table-to-text generation, automated evaluation, and feedback generation, respectively. Experimental results indicate that the current high-performing LLM, specifically GPT-4, can effectively serve as a table-to-text generator, evaluator, and feedback generator, facilitating users' information seeking purposes in real-world scenarios. However, a significant performance gap still exists between other open-sourced LLMs (e.g., Tulu and LLaMA-2) and GPT-4 models. Our data and code are publicly available at https://github.com/yale-nlp/LLM-T2T.

==> figures/dataset_example.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth]{figures/figures/LOTNLG.png}
    \caption{An example of \lotnlg, where models are required to generate statements using the specified types of logical reasoning operations}
    \label{fig:lotnlg_example}
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width = \linewidth]{figures/figures/f2wtq_example.pdf}
    \caption{An example of \wtqnew, where models need to perform human-like reasoning to generate response.}
    \label{fig:wtqnew_example}
\end{figure}
